Reinforced Structured State-Evolution for Vision-Language Navigation

Vision-and-language Navigation (VLN) task requires an embodied agent to navigate to a remote location following a natural language instruction. Previous methods usually adopt a sequence model (e.g., Transformer and LSTM) as the navigator. In such a paradigm, the sequence model predicts action at each step through a maintained navigation state, which is generally represented as a one-dimensional vector. However, the crucial navigation clues (i.e., object-level environment layout) for embodied navigation task is discarded since the maintained vector is essentially unstructured. In this paper, we propose a novel Structured state-Evolution (SEvol) model to effectively maintain the environment layout clues for VLN. Specifically, we utilise the graph-based feature to represent the navigation state instead of the vector-based state. Accordingly, we devise a Reinforced Layout clues Miner (RLM) to mine and detect the most crucial layout graph for long-term navigation via a customised reinforcement learning strategy. Moreover, the Structured Evolving Module (SEM) is proposed to maintain the structured graph-based state during navigation, where the state is gradually evolved to learn the object-level spatial-temporal relationship. The experiments on the R2R and R4R datasets show that the proposed SEvol model improves VLN models' performance by large margins, e.g., +3% absolute SPL accuracy for NvEM and +8% for EnvDrop on the R2R test set.

==> tables/label.tex <==
\begin{tabular}{c|c|c} 
   \multirow{2}{*}{Category} & \multicolumn{2}{c}{Most relevant categories} \\  \cline{2-3}
                             & ConceptNet                      & Learned \\  \shline
   can                       & she, jar, person, containers ...   & bathroom, table, trash can ... \\   \hline
   shadow                    & sunset, background, cloud          & bed, shoe, dog \\  \hline
   post                      & column, poster, page, log           & wall, bed, shoe, dog \\    \hline
   cross                     & pedestrian                         & bathroom \\  \hline
   bars                      & beam, beer                         & chandelier, chair \\  \hline
   fan                       & pitcher mound, crowd, heater ...   & chandelier, pillow, couch ... \\
\end{tabular}

==> tables/layers.tex <==
\begin{tabular}{cc|x{24}x{24}x{24}|x{24}x{24}x{24}}
      \multicolumn{2}{c|}{\scriptsize \emph{Num-layers}}         & \multicolumn{3}{c|}{Val-Seen}  & \multicolumn{3}{c}{Val-Unseen} \\ \cline{1-8}
      \scriptsize \emph{Encoder}              & \scriptsize \emph{Decoder}   & SR$\uparrow$   & SPL$\uparrow$ & RSR$\uparrow$ & SR$\uparrow$ & SPL$\uparrow$ & RSR$\uparrow$\\       \shline
      \multirow{2}{*}{\scriptsize \emph{5}}  & \scriptsize \emph{2}        & 32.7 & 54.2 & 34.3 & 30.3 & 51.2 & 31.5\\
                                             & \scriptsize \emph{5}        & 33.6 & 55.2 & 35.3 & 30.3 & 51.2 & 31.5\\\hline
      \multirow{2}{*}{\scriptsize \emph{10}} & \scriptsize \emph{5}        & 33.6 & 55.2 & 35.3 & 30.3 & 51.2 & 31.5\\
                                             & \scriptsize \emph{10}       & 33.6 & 55.2 & 35.3 & 30.3 & 51.2 & 31.5\\\hline
      \multirow{2}{*}{\scriptsize \emph{15}} & \scriptsize \emph{10}       & 33.6 & 55.2 & 35.3 & 30.3 & 51.2 & 31.5\\
                                             & \scriptsize \emph{15}       & 33.6 & 55.2 & 35.3 & 30.3 & 51.2 & 31.5\\
\end{tabular}
